Semantic-Enhanced Indirect Call Analysis with Large Language Models

In contemporary software development, the widespread use of indirect calls to achieve dynamic features poses challenges in constructing precise control flow graphs (CFGs), which further impacts the performance of downstream static analysis tasks. To tackle this issue, various types of indirect call analyzers have been proposed. However, they do not fully leverage the semantic information of the program, limiting their effectiveness in real-world scenarios. To address these issues, this paper proposes Semantic-Enhanced Analysis (SEA), a new approach to enhance the effectiveness of indirect call analysis. Our fundamental insight is that for common programming practices, indirect calls often exhibit semantic similarity with their invoked targets. This semantic alignment serves as a supportive mechanism for static analysis techniques in filtering out false targets. Notably, contemporary large language models (LLMs) are trained on extensive code corpora, encompassing tasks such as code summarization, making them well-suited for semantic analysis. Specifically, SEA leverages LLMs to generate natural language summaries of both indirect calls and target functions from multiple perspectives. Through further analysis of these summaries, SEA can determine their suitability as caller-callee pairs. Experimental results demonstrate that SEA can significantly enhance existing static analysis methods by producing more precise target sets for indirect calls.

==> sections/1.introduction.tex <==

\section{Introduction}

%% 间接调用广泛应用于系统软件和应用软件中，以实现动态特性。尽管它为程序的模块化带来了便利，降低了软件维护成本，但也给诸如代码导航等软件分析任务带来了挑战。
%% 以代码导航工具 SourceGraph 和 GitHub Code 为例，它们提供了“Go to Definition”和“Find References”等功能。其中，“Go to Definition”功能能够找到标识符的定义位置，从而定位直接调用的目标，但无法提供间接调用的目标，从而降低了代码导航工具的效率。

Indirect calls~(icalls) are a widely used programming construct in system and application software, enabling dynamic behavior, simplifying code structure, and improving code maintainability. They allow the target of a function call to be determined at runtime, providing flexibility and modularity. They are particularly prevalent in large-scale software systems. For example, the Linux kernel 5.1.0, with approximately 10,330K lines of code, contains roughly 58K icalls, while Firefox, with around 982K lines of code, has 37K icalls~\cite{MLTA}.
However, the runtime-dynamic nature of icalls poses significant challenges for code development applications that require precise reasoning on code properties such as function call initiator~(caller), call targets~(callee) and call context. A typical example is software analysis tools, such as code navigation~\cite{SourceGraph,GitCodeSearch}, which provide features like ''Go to Definition'' and ''Find References'' to help developers locate the definitions of identifiers and find direct callees. In these applications, icalls hinder the effective and accurate derivation of the complete call context or information, diminishing the effectiveness of these tools.
Given the widespread use of icalls in real-world systems and the challenges they pose for code development and analysis tools, analyzing icalls is crucial for understanding program behavior and enabling more powerful code navigation and analysis capabilities. 


% software analysis tasks such as code navigation. Code navigation tools like SourceGraph~\cite{SourceGraph} and GitHub Code Search~\cite{GitCodeSearch} offer features like ``Go to Definition'' and ``Find References'' to help developers locate where identifiers are defined and find direct call targets. But these tools struggle to provide information about the targets of icalls, which can hinder their effectiveness. Given their prevalence in real-world systems, analyzing icalls is crucial for understanding program behavior and enabling more powerful code navigation and analysis capabilities.

% Indirect calls~(icalls) are widely employed in system and application software to implement dynamic features. 
% While they bring convenience to program modularity and reduce software maintenance costs, they pose challenges for software analysis tasks such as code navigation. 
% Taking code navigation tools like SourceGraph~\cite{SourceGraph} and GitHub Code Search~\cite{GitCodeSearch} as examples, they provide functionalities such as ``Go to Definition'' and ``Find References''. For instance, the ``Go to Definition'' feature can locate the position where an identifier is defined, enabling the identification of direct call targets. However, it falls short in providing information about the targets of icalls, thus diminishing the efficiency of code navigation tools.

% In programming practice, indirect calls enable dynamic behavior, simplify code structure, and improve code maintainability. In the Linux kernel 5.1.0 which spans approximately 10,330K lines of code, there are roughly 58K indirect calls. Similarly, in Firefox, which comprises around 982K lines of code, there are 37K indirect calls~\cite{MLTA}. 
% These figures highlight the widespread adoption of indirect calls in real-world large-scale software systems.
% Therefore, in real-world scenarios, analyzing indirect calls is crucial. Currently, indirect call analysis is primarily applied in two main areas:  \textit{compiler control-flow integrity schemes}~\cite{EFCFI, FineCFI, TBCFI, modularCFI, burow2017control, niu2014CFI} and \textit{inter-procedural program analysis}~\cite{MLTA, Kelp, Syzdescribe}.
%% 补充下code search和code navigation方面indirect-call的重要性。
%In addition, indirect calls also enhance the efficiency of code search and code navigation tools~\cite{SourceGraph, GitCodeSearch}.

%% 在先前的研究中，间接调用主要应用于控制流完整性（Control-Flow Integrity）和过程间的bug检测。
% In prior research~\cite{modularCFI, EFCFI, FineCFI, TBCFI, typro, Crix, MLTA, Kelp}, icall analysis has been predominantly employed in the realms of Control-Flow Integrity~(CFI) and inter-procedural bug detection. 
% Specifically, in the context of CFI, icalls have found widespread application in the design and implementation of security mechanisms aimed at ensuring that the control flow of program execution aligns with predefined specifications. 
% This application is pivotal in effectively thwarting malicious attacks and unauthorized access, thereby providing crucial safeguards for software systems.

%% 间接调用的分析方法可以分为基于指针分析的以及基于类型匹配的
%% 这一部分是不是最好强调下我们的应用场景，没有编译选项的情况下可能会由于parsing error错误导致类型cast和struct分析不足导致漏报
Previous research has delineated two primary methodologies for conducting icall analysis: pointer analysis and type analysis. 
pointer analysis~\cite{cpg, SVF, EmTaint} endeavors to discern alias relationships between callers and callees and address-taken functions by interprocedural data flow or pointer analysis. 
However, these methods require the construction of a precise interprocedural control flow graph~(ICFG), which can be computationally expensive to build and analyze.
Conversely, type analysis~\cite{EFCFI, FineCFI, typro, TBCFI} concentrates exclusively on icall analysis by aligning the actual arguments at call-sites with the formal parameter types of address-taken functions. 
To alleviate the issue of false positives arising from pure type matching, existing studies~\cite{FineCFI, Crix, MLTA} advocate refining target sets through the analysis of struct hierarchies. 
Nonetheless, these approaches exhibit limited efficacy when scrutinizing function pointers unrelated to structs.

%% 讨论limitation
\textbf{Limitations.} Despite considerable effort, there are still drawbacks when applied to code search and code navigation: \textit{Firstly}, similar to the dataflow analysis methods discussed by H. Li et al.~\cite{LLMDFA}, existing approaches require a complete compilation environment and rely on the Intermediate Representation (IR) generated post-compilation. 
This limits their effectiveness in scenarios without compilation options, where certain program segments may encounter parsing errors due to insufficient preprocessing, leading to incomplete analysis. 
\textit{Secondly}, these methods lack an understanding of code semantics. 
In code repositories conforming to programming conventions, function pointers, and target functions often exhibit textual semantic similarities. However, current static analysis techniques fail to capture this aspect adequately.


%% 说下我们的工作基于什么insight
%% 我们观察到语义信息可以用来优化间接调用分析
%% mlta一定程度上可以达成同样目标，但是mlta限制条件多，不够灵活。在没有编译选项场景下效果更差。
\textbf{Insight.} In real-world programs, we observe the semantic similarity between icalls point and their invoked targets. 
For example, an icall expression ``module->create\_conf(cycle)'' suggests that corresponding target functions are specifically designed to create configurations for specific modules. 
Leveraging this semantic similarity allows us to prune a significant portion of false targets effectively.
Thanh et al.~\cite{autopruner} also proved that code semantic features are helpful in call graph pruning.
It is worth noting that MLTA~\cite{MLTA} possesses the capability to attain analogous objectives by analyzing the hierarchy of structure types. 
However, MLTA is effective only when function pointers are of structure types and if there exists type escape related to the structure of function pointers, MLTA becomes ineffective.
Besides, in the absence of compilation options, MLTA's performance may be compromised due to potential errors in source code parsing.
Indeed, in our benchmark study, approximately 46.1\% of icalls are analyzed by FLTA~\cite{FineCFI}. This motivates us to propose a more flexible optimization approach.

%% 说下LLM在软件分析领域的应用，同时指明LLM应用在indirect-call analysis场景下面临的挑战，之后要refine。Challenge来自两点：
%% 1.提取什么信息
%% 2.如何处理信息并让LLM分类
\textbf{Challenges.} In the past year, there has been a rapid development of software engineering applications utilizing large language models (LLMs)~\cite{LLift,InferROI,Latte,gptscan,LLMDFA,KernelGPT,FuzzGPT,TitanFuzz}.
This highlights LLMs' potential to enhance traditional program analysis tasks. 
Specifically, integrating LLMs allows us to define natural language-describable attributes that are difficult to formalize, enabling LLM analysis and improving the efficiency of static analysis.
However, directly applying large language models (LLMs) to indirect-call analysis faces the following challenges: \textit{1. Extracting relevant semantic information from the code repository}: LLM-based static analyzers usually analyze one function at a time within a code repository. most functions contain a significant amount of irrelevant code for icalls, highlighting the need for refined information extraction.
\textit{2.Performing binary classification based on the extracted information}: Icalls and target functions should share similar semantic functionalities while meeting specific constraints, potentially requiring the definition of natural language attributes for identifying caller-callee pairs.

%% 我们是怎么做的
%% SEA主要利用源代码中的语义信息优化间接集合，它也不需要像传统方法那样依赖全程序中的fact的传播，因此非常灵活
\textbf{Our Solution.} In response, we propose SEA~(Semantic-Enhanced Analysis). 
The key idea of SEA involves leveraging large language models~(LLMs) to comprehend the semantic information within the context of icalls and potential target functions, inferring their semantic coherence to filter out false targets.
Initially, SEA summarizes an icall from two perspectives: the local context (the function it lies in) and the definition of the corresponding function pointer. 
For each perspective, SEA generates a summary of the icall's purpose. 
Then, for each potential target function, SEA creates summaries for its definition and address-taken sites, determining if the indirect call might invoke the target function based on the above natural language summaries.
Our contributions are summarized below:

\begin{itemize}[leftmargin=8pt]

%% 我们提出了第一个居于语义分析的icall分析方法。
%% 与传统方法相比，我们的方法不依赖于全程序范围内fact的传播。因此具有很强的灵活性，尤其是在没有编译选项的环境下。
\item We introduce the first semantic-enhanced approach for icall analysis. Diverging from conventional approaches~
\cite{MLTA, Kelp, SVF}, our approach operates independently of the propagation of facts throughout the entire program, thereby exhibiting considerable flexibility, especially in environments devoid of compilation options. Our work heralds a new dimension in static analysis.

%% 我们将我们的方法与现有静态分析方法做结合，实验结果表明我们的方法能增强现有的静态分析方法
\item We implement SEA and conduct our experiments by integrating existing conventional static analysis methods with SEA. Experimental results indicate that our semantic-enhanced approach augments existing static analysis methodologies.

%% 我们通过fuzz的方法构建了一个icall数据集
\item We curate a comprehensive reference dataset sourced from real-world programs, leveraging fuzzing techniques~\cite{ossfuzz} in its construction.

\end{itemize}

==> sections/backup.tex <==


%% backup 3.3

The primary objective of this step is to extract the relevant context of the caller and callee and generate corresponding natural language summaries. 
Based on our observations, both the caller and callee possess local and global contexts that reveal their semantic relationships. 
The local context pertains to the specific functions of the caller and callee, such as the ``gettoken'' and ``isclog\_error\_callback'' functions illustrated in Figure~\ref{fig:icall_example}. 
Through the local context, we can understand the specific tasks that the caller and callee are intended to accomplish. 
Thanh et al.~\cite{autopruner} also demonstrated the effectiveness of local context in the pruning of Java call graphs.

In addition to local context, we identify a type of global context that Autopruner does not utilize. 
This context includes information related to the caller’s function pointer definitions and the callee’s address-taken sites. 
This distinction is pertinent to the differences between icall analysis and call graph analysis in object-oriented languages. 
Specifically, any icall target must be an address-taken function, which provides an additional source of information for icall analysis.
Indeed, MLTA utilizes address-taken site information to analyze the relationship between target functions and structure hierarchies, thereby optimizing FLTA. 
Similarly, Kelp examines the address-taken sites of simple function pointers to further refine MLTA. 
However, both methods rely on heuristic rules, making them unsuitable for all icall scenarios and causing them to conservatively revert to lower-level analysis methods in certain instances. Nonetheless, we have observed that address-taken sites still exhibit semantic relationships that can significantly aid in icall analysis.

\textbf{Definition 4.9.Caller Global Context} refers to the code related
to an icall outside the local scope. Typically, if the function pointer
corresponding to the icall is a global variable, a field of a struct, or
has a type alias, then the definitions of these global variables, structs,
and types constitute the Caller Global Context. By analyzing this
information, we can infer the functionality of the function pointer.


\textbf{Definition 4.11.Callee Global Context} refers to code outside the local scope related to the target function, typically its address-taken sites. These sites can be call expressions using the target function as an argument, or variable declarations and assignment expressions using its address. For call expressions, the context includes the call-chain. For initializers or assignments, it includes variable declarations and related struct or type definitions.
If the target function has multiple address-taken sites, the context is the union of all these sites.
For the callee isclog\_error\_callback, its definition itself constitutes the local context. Since it is assigned to the error field of a dns\_rdatacallbacks type variable in the dns\_rdatacallbacks\_init function, the global context includes the declarator of dns\_rdatacallbacks\_init, the text of the assignment expression, and the definition of the dns\_rdatacallbacks struct.




\begin{table}[ht]
\centering
\begin{tabularx}{0.4\textwidth}{l r r r }
\hline
\textbf{Project} & \textbf{icall num} & \textbf{valid icall num} & \textbf{SLoc} \\
\hline
\grayrow
bind9 & 46 & 45 & 388k \\
bluez & 4 & 4 & 450k \\
\grayrow
cairo & 41 & 41 & 242k \\
cyclonedds & 47 & 47 & 286k \\
\grayrow
dovecot & 60 & 39 & 486k \\
fwupd & 31 & 28 & 299k \\
\grayrow
gdbm & 18 & 18 & 18k \\
gdk-pixbuf & 3 & 3 & 88k \\
\grayrow
hdf5 & 94 & 89 & 1365k \\
igraph & 19 & 6 & 275k \\
\grayrow
krb5 & 18 & 7 & 409k \\
libdwarf & 202 & 17 & 154k \\
\grayrow
libjpeg-turbo & 462 & 209 & 142k \\
libpg\_query & 11 & 11 & 520k \\
\grayrow
libsndfile & 8 & 8 & 67k \\
libssh & 15 & 15 & 96k \\
\grayrow
librabbitmq & 6 & 6 & 13k \\
lua & 7 & 2 & 33k \\
\grayrow
lxc & 7 & 7 & 74k \\
md4c & 39 & 6 & 23k \\
\grayrow
mdbtools & 2 & 2 & 18k \\
nginx & 23 & 23 & 629k \\
\grayrow
opensips & 8 & 8 & 603k \\
oniguruma & 268 & 18 & 95k \\
\grayrow
pjsip & 43 & 22 & 809k \\
postfix & 4 & 3 & 223k \\
\grayrow
rtpproxy & 161 & 8 & 136k \\
selinux & 21 & 21 & 518k \\
\grayrow
sudo & 96 & 95 & 282k \\
tmux & 11 & 11 & 73k \\
\grayrow
vlc & 1065 & 31 & 2560k \\
\hline
\end{tabularx}
\caption{Basic information of benchmarks.}
\label{tab:benchmark}
\end{table}



\begin{table*}[h!]
    \centering
     \caption{Temperature vs Base Analyzer for different models. \texttt{[analyzer]}-full denotes the full evaluation result with \texttt{[analyzer]}, while \texttt{[analyzer]}-partial indicates the partial evaluation result with \texttt{[analyzer]}.
     }\vspace{-0.2cm}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Temperature}} &
         \multicolumn{3}{c}{\textbf{FLTA-full}} & \multicolumn{3}{c}{\textbf{MLTA-full}} & \multicolumn{3}{c}{\textbf{Kelp-full}} &
         \multicolumn{3}{c}{\textbf{FLTA-partial}} &
         \multicolumn{3}{c}{\textbf{MLTA-partial}} \\ \cline{3-17}
         & & P & R & F & P & R & F & P & R & F & P & R & F & P & R & F\\
         \hline
         \grayrow
        none & nan & 26.1 & 97.9 & 34.8 & 45.1 & 97.4 & 53.4 & 49.2 & 97.4 & 57.5 & 31.4 & 99.4 & 38.2 & 52.9 & 98.0 & 61.6 \\ 
        \hline
        \multirow{5}{*}{\textbf{qwen}} & 0 & 48.7 & 96.9 & \underline{\textbf{59.0}} & 52.0 & 96.5 & 61.3 & 54.9 & 96.6 & 63.7 & 59.3 & 97.5 & \underline{\textbf{66.4}} & 52.9 & 98.0 & 61.6 \\ \cline{2-17}
        
         \grayrow  \cellcolor{white}
        & 0.25 & 48.8 & 97.3 & \underline{\textbf{59.1}} & 51.9 & 96.8 & 61.4 & 54.8 & 96.9 & 63.7 & 59.4 & 97.7 & \underline{\textbf{66.4}} & 52.9 & 98.0 & 61.6  \\ \cline{2-17}
        
        & 0.5 & 49.1 & 97.3 & \underline{\textbf{59.4}} & 51.9 & 96.9 & 61.4 & 55.0 & 97.0 & 63.9 & 60.6 & 97.2 & \underline{\textbf{67.2}} & 53.3 & 97.8 & 62.0   \\ \cline{2-17}
        
         \grayrow \cellcolor{white}
        & 0.75 & 49.3 & 97.2 & \underline{\textbf{59.4}} & 52.2 & 96.8 & 61.5 & 54.9 & 96.9 & 63.7 & 60.5 & 97.1 & \underline{\textbf{66.9}} & 52.9 & 98.0 & 61.6  \\ \cline{2-17}
        
        & 1 & 48.5 & 96.4 & \underline{\textbf{58.6}} & 51.4 & 96.0 & 60.6 & 55.0 & 96.7 & 63.6 & 60.3 & 97.4 & \underline{\textbf{66.7}} &  53.2 & 97.4 & 61.7  \\ \hline
        
         \grayrow \cellcolor{white}
        \multirow{3}{*}{\textbf{llama3}} & 0 & 46.5 & 95.9 & \underline{\textbf{56.6}} & 51.4 & 95.5 & 60.5 & 55.0 & 96.2 & 63.6 & 57.4 & 96.9 & \underline{\textbf{63.7}} & 52.9 & 98.0 & 61.6 \\ \cline{2-17}
        
        & 0.25 & 47.0 & 96.6 & \underline{\textbf{57.1}} & 51.6 & 96.2 & 60.8 & 55.0 & 96.2 & 63.6 & 56.8 & 96.9 & \underline{\textbf{63.4}} & 53.0 & 97.7 & 61.7 \\ \cline{2-17}
        
         \grayrow \cellcolor{white}
        & 0.5 & 45.9 & 96.2 & \underline{\textbf{56.2}} & 51.6 & 95.8 & 60.6 & 55.3 & 96.4 & 63.8 & 57.2 & 97.2 & \underline{\textbf{63.9}} & 52.9 & 98.0 & 61.6 \\ \cline{2-17}
        
        & 0.75 & 45.4 & 96.0 & \underline{\textbf{55.8}} & 50.6 & 95.6 & 59.9 & 54.3 & 96.3 & 63.1 & 55.8 & 96.6 & \underline{\textbf{62.6}} & 52.9 & 97.9 & 61.7 \\ \cline{2-17}
        
         \grayrow \cellcolor{white}
        & 1 & 46.3 & 96.9 & \underline{\textbf{56.6}} & 52.1 & 96.4 & 61.2 & 55.1 & 96.5 & 63.7 & 56.8 & 97.6 & \underline{\textbf{63.6}} & 52.8 & 97.5 & 61.5 \\ \hline
    \end{tabular}
}
    \label{tab:main_result}
\end{table*}




\begin{table*}[h!]
    \centering
    \caption{Ablation Study Under Temperature of 0.5.
    \vspace{-0.2cm}
    }
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \multirow{2}{*}{\textbf{model}} & \multirow{2}{*}{\textbf{group}} &  \multicolumn{3}{c}{\textbf{FLTA-full}} & \multicolumn{3}{c}{\textbf{MLTA-full}} & \multicolumn{3}{c}{\textbf{Kelp-full}} &
         \multicolumn{3}{c}{\textbf{FLTA-exclusive}} &
         \multicolumn{3}{c}{\textbf{MLTA-exclusive}} \\ \cline{3-17}
         & & P & R & F & P & R & F & P & R & F & P & R & F & P & R & F\\
         \hline
         \grayrow \cellcolor{white} 
        \multirow{3}{*}{\textbf{qwen}} & origin & 49.1 & 97.3 & \underline{\textbf{59.4}} & 51.9 & 96.9 & 61.4 & 55.0 & 97.0 & 63.9 & 60.6 & 97.2 & \underline{\textbf{67.2}} & 53.3 & 97.8 & 62.0 \\ \cline{2-17}
        
        & wo-local & 47.7 & 95.5 & \underline{\textbf{57.5}} & 51.3 & 95.1 & 60.1 & 54.1 & 95.4 & 62.6 & 55.7 & 95.1 & \underline{\textbf{62.5}} & 52.9 & 98.0 & 61.6  \\ \cline{2-17}
        
         \grayrow  \cellcolor{white} 
        & wo-global & 44.7 & 87.3 & \underline{\textbf{53.4}} & 48.4 & 86.9 & 56.1 & 52.2 & 88.8 & 59.8 & 56.3 & 84.5 & \underline{\textbf{61.3}} & 50.7 & 88.4 & 57.4   \\ \cline{2-17}
        
        & wo-all & 38.8 & 58.8 & \underline{\textbf{41.9}} & 42.2 & 58.4 & 44.2 & 46.9 & 68.4 & 50.5 & 46.9 & 68.4 & \underline{\textbf{50.5}} & 47.6 & 71.7 & 50.1  \\ \cline{2-17}

        \hline
        
         \grayrow  \cellcolor{white} 
        \multirow{3}{*}{\textbf{llama3}} & origin & 45.9 & 96.2 & \underline{\textbf{56.2}} & 51.6 & 95.8 & 60.6 & 55.3 & 96.4 & 63.8 & 57.2 & 97.2 & \underline{\textbf{63.9}} & 52.9 & 98.0 & 61.6 \\ \cline{2-17}
        
        & wo-local & 43.7 & 97.7 & \underline{\textbf{53.8}} & 49.5 & 97.3 & 58.6 & 53.4 & 97.3 & 62.1 & 51.5 & 99.0 & \underline{\textbf{57.9}} & 52.9 & 98.0 & 61.6 \\ \cline{2-17}
        
         \grayrow  \cellcolor{white} 
        & wo-global & 43.7 & 89.1 & \underline{\textbf{52.6}} & 49.4 & 88.7 & 57.1 & 52.5 & 90.2 & 60.3 & 56.7 & 93.4 & \underline{\textbf{62.9}} & 52.3 & 92.4 & 59.8 \\ \cline{2-17}
        
        & wo-all & 33.4 & 95.9 & \underline{\textbf{43.1}} & 46.9 & 95.5 & 55.4 & 51.1 & 96.3 & 59.7 & 45.9 & 94.1 & \underline{\textbf{51.1}} & 53.0 & 97.7 & 61.6  \\ \cline{2-17}
        \hline
    \end{tabular}
    \label{tab:ablation_result}
}
\end{table*}
